Adaptive Controllers for Quadrotors Carrying Unknown Payloads

With the advent of intelligent transport, quadrotors are becoming an attractive solution while lifting or dropping payloads during emergency evacuations, construction works, etc. During such operations, dynamic variations in (possibly unknown) payload cause considerable changes in the system dynamics. However, a systematic control solution to tackle such varying dynamical behaviour is still missing. In this work, two control solutions are proposed to solve two specific problems in aerial transportation of payload, as mentioned below. In the first work, we explore the tracking control problem for a six degrees-of-freedom quadrotor carrying different unknown payloads. Due to the state-dependent nature of the uncertainties caused by variation in the dynamics, the state-of-the-art adaptive control solutions would be ineffective against these uncertainties that can be completely unknown and possibly unbounded a priori. In addition, external disturbances such as wind while following a trajectory in all three positions and attitude angles. Hence, an adaptive control solution for quadrotors is proposed, which does not require any a priori knowledge of the parameters of quadrotor dynamics and external disturbances. The second work is focused on the interchanging dynamic behaviour of a quadrotor while loading and unloading different payloads during vertical operations. The control problem to maintain the desired altitude is formulated via a switched dynamical framework to capture the interchanging dynamics of the quadrotor during such vertical operations, and a robust adaptive control solution is proposed to tackle such dynamics when it is unknown. The stability of the closed-loop system is studied analytically and the effectiveness of the proposed solution is verified via simulations.

==> LaTex/control_system.tex <==

A control system is used to establish a bridge between what we have (current outputs) and what we need (setpoints or desired outputs). It is mainly classified into two types: open-loop and closed-loop. An open-loop control system is a direct mapping between expected outputs and desired control inputs. This mapping is defined as the dynamics of the robotic system or commonly mentioned as a plant.

A feedback element is added in a closed-loop control system to compensate for any error in the mapping. The block diagram Fig: \ref{fig:closed_loop} represents a closed-loop control system. As mentioned earlier, the plant represents the dynamics of the robot. It consists of one or more actuators to perform a given task. A controller receives the error signal, which is the difference between the expected output and the obtained output. Based on the error signal, the controller gives out a control signal (or the actuator signal) to set the actuators to a particular value. A feedback element is a set of sensors that measure the current output and send the feedback signal to the error block.


\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{LaTex/figures/control_system.jpg}%{FIG5_16-TIE-3042.eps}
	\caption{{A schematic representing a closed-loop control system.}}\label{fig:closed_loop}
\end{figure}


Conventionally the controller has to be aware of the dynamics of the robotic system to generate an appropriate actuator signal for a given setpoint. Hence the dynamics of the robot has to be modelled mathematically using forces and torques. The commonly used way of modelling a mechanical system (robot) is using Euler-Lagrangian dynamics.
